On Erlang ODE approximations of differential equations with distributed time delays

In this paper, we propose a general approach for approximate simulation and analysis of delay differential equations (DDEs) with distributed time delays based on methods for ordinary differential equations (ODEs). The key innovation is that we 1) propose an Erlang mixture approximation of the kernel in the DDEs and 2) use the linear chain trick to transform the resulting approximate DDEs to ODEs. We refer to this as the Erlang ODE approximation of the DDEs, and we prove that the Erlang mixture approximation converges for continuous and bounded kernels if the number of terms increases sufficiently fast. Furthermore, we show that if the kernel is also exponentially bounded, the Erlang ODE approximation can be used to assess the stability of the steady states of the original DDEs and that the solution to the ODE approximation converges. Additionally, we propose an approach based on bisection and least-squares estimation for determining optimal parameter values in the approximation. Finally, we present numerical examples that demonstrate the accuracy and convergence rates of the approximations and the efficacy of the proposed approach for bifurcation analysis and Monte Carlo simulation. The numerical examples involve a modified logistic equation, chemotherapy-induced myelosuppression, and a point reactor kinetics model of a molten salt nuclear fission reactor.

==> tex/linear_chain_trick.tex <==
\section{Approximate system of ordinary differential equations}\label{sec:lct}
In this section, we use the Erlang mixture approximation presented in Section~\ref{sec:approx} to approximate the multivariate kernel in the DDEs presented in Section~\ref{sec:system}, and we use the LCT to transform the resulting approximate system to ODEs. Furthermore, we describe the steady state equations for the approximate system of ODEs together with a stability criterion\chg{, and we use Hurwitz' convergence theorem to show that the \chgtwo{isolated} roots of the characteristic function for the original system of DDEs are accumulation points for the roots of the characteristic function for the approximate system of ODEs. Finally, we analyze the stability of the state error dynamics, and we use the theorem presented by Guglielmi and Hairer~\cite{Guglielmi:Hairer:2025} to prove that the solution to the approximate system of ODEs converges to that of the original system.}

First, we approximate the system of DDEs~\eqref{eq:system:x}--\eqref{eq:system:delay} by
%
\begin{subequations}\label{eq:lct:approximate:system:DDE}
	\begin{align}
		\label{eq:lct:approximate:system:DDE:x}
		\dot{\hat x}(t) &= f(\hat x(t), \hat z(t)), \\
		%
		\label{eq:lct:approximate:system:DDE:z}
		\hat z(t) &= \int\limits_{-\infty}^t \hat \alpha(t - s) \odot \hat r(s) \incr s, \\
		%
		\label{eq:lct:approximate:system:DDE:r}
		\hat r(t) &= h(\hat x(t)),
	\end{align}
\end{subequations}
%
where each element of the kernel $\hat \alpha: \Rnn^{n_z} \rightarrow \R^{n_z}$ is an Erlang mixture \chgtwo{approximation of $\alpha_i$ (see Proposition~\ref{thm:erlang:mixture:approximation})}:
%
\begin{align}\label{eq:lct:approximate:kernel:DDE}
	\hat \alpha_i(t) &= \sum_{m=0}^{M_i} c_{m, i} \ell_{m, i}(t), & i &= 1, \ldots, n_z.
\end{align}
%
The subscript $i$ on the Erlang kernels, $\ell_{m, i}: \Rnn \rightarrow \Rnn$, indicates that it depends on the $i$'th rate parameter, $a_i \in \Rp$. Furthermore, $\hat x: \R \rightarrow \R^{n_x}$ and $\hat z, \hat r: \R \rightarrow \R^{n_z}$ are approximations of $x$, $z$, and $r$, respectively.

\begin{proposition}[\chgtwo{Linear chain trick}]\label{thm:linear:chain:trick}
	The system of DDEs~\eqref{eq:lct:approximate:system:DDE} with the kernel~\eqref{eq:lct:approximate:kernel:DDE} is equivalent to the system of ODEs
	%
	\begin{subequations}\label{eq:lct:approximate:system:ODE}
		\begin{align}
			\label{eq:system:approximate:x}
			\dot{\hat x}(t) &= f(\hat x(t), \hat z(t)), \\
			%
			\label{eq:system:approximate:Z}
			\dot{\hat Z}(t) &= A \hat Z(t) + B \hat r(t), \\
			%
			\label{eq:system:approximate:z}
			\hat z(t) &= C \hat Z(t), \\
			%
			\hat r(t) &= h(\hat x(t)),
		\end{align}
	\end{subequations}
	%
	where $\hat Z: \R \rightarrow \R^{M + n_z}$ contains auxiliary memory states, and $M = \sum_{i=1}^{n_z} M_i$. Furthermore, the matrices $A\in \R^{M + n_z \times M + n_z}$, $B \in \Rnn^{M + n_z \times n_z}$, \chg{and} $C \in \chmtwo{\R}^{n_z \times M + n_z}$ are block-diagonal:
	%
	\begin{subequations}
		\begin{align}
			A &= \blkdiag\left(A^{(1)}, A^{(2)}, \ldots, A^{(n_z)}\right), \\
			B &= \blkdiag\left(b^{(1)}, b^{(2)}, \ldots, b^{(n_z)}\right), \\
			C &= \blkdiag\left(c^{(1)}, c^{(2)}, \ldots, c^{(n_z)}\right).
		\end{align}
	\end{subequations}
	%
	The block-diagonal elements, $A^{(i)} \in \R^{(M_i+1) \times (M_i+1)}$, $b^{(i)} \in \Rnn^{M_i+1 \times 1}$, and $c^{(i)} \in \chmtwo{\R}^{1 \times M_i+1}$, are given by
	%
	\begin{subequations}
		\begin{align}
			A^{(i)} &= a_i (L^{(i)} - I^{(i)}), &
			b^{(i)} &= a_i e_1^{(i)}, &
			c^{(i)} &=
			\begin{bmatrix}
				c_{0, i} & c_{1, i} & \cdots & c_{M_{i}, i}
			\end{bmatrix}, & i &= 1, \ldots, n_z,
		\end{align}
	\end{subequations}
	%
	where $I^{(i)}, L^{(i)} \in \R^{M_i+1 \times M_i+1}$ are an identity matrix and a lower shift matrix, respectively, i.e., $L^{(i)}$ contains ones in the first subdiagonal and zeros elsewhere. Furthermore, the first element of $e_1^{(i)} \in \R^{M_i+1 \times 1}$ is one and the others are zero.
\end{proposition}
%
The transformation of the system of DDEs~\eqref{eq:lct:approximate:system:DDE} to the system of ODEs~\eqref{eq:lct:approximate:system:ODE} is standard~\cite{MacDonald:1978, Ponosov:etal:2004}. Therefore, we postpone the proof of \chgtwo{Proposition}~\ref{thm:linear:chain:trick} to Appendix~\ref{sec:deriv}.

\input{./tex/steady_states_and_stability}
\input{./tex/convergence_of_the_roots}
\input{./tex/error_dynamics}


==> tex/linearized_stability.tex <==
\section{\chgtwo{Prerequisites of stability criterion}}\label{sec:linearized:stability}
\chgtwo{In this section, we verify that the system~\eqref{eq:system}--\eqref{eq:system:delay} satisfies the conditions of Theorem~4.7 in the paper by Diekmann and Gyllenberg~\cite{Diekmann:Gyllenberg:2012}.}

\chgtwo{We express the linearized system~\eqref{eq:linearized:system} as
%
\begin{align}
	\dot X(t) &= \int_0^\infty \mu(\mathrm ds) X(t - s),
\end{align}
%
where $\mu$ is a measure with a density given by
%
\begin{align}
	\eta(s) &= F \delta(s) + G \alpha(s) H.
\end{align}
%
Here, $\delta$ is Dirac's delta and the matrices $F$, $G$, and $H$ are given by~\eqref{eq:jacobians}. The linearized system~\eqref{eq:linearized:system} can be derived from the above equation by
%
\begin{align}
	\dot X(t)
	&= \int_0^\infty \mu(\mathrm ds) X(t - s) = \int_0^\infty \eta(s) X(t - s) \incr s \\
	&= \int_0^\infty (F \delta(s) + G \alpha(s) H) X(t - s) \incr s \nonumber \\
	&= F \int_0^\infty \delta(s) X(t - s) \incr s + G \int_0^\infty \alpha(s) H X(t - s) \incr s \nonumber \\
	&= F X(t) + G \int_{-\infty}^t \alpha(t - s) H X(s) \incr s. \nonumber
\end{align}
}%

\chgtwo{Let $\varrho \in \Rp$ be given such that $\sigma < \varrho < \rho$ where $\sigma$ is the rate parameter in the exponential bound of the initial state function, $x_0$, and $\rho$ is the smallest rate parameter in the exponential bounds on the elements of the kernel $\alpha$. Diekmann and Gyllenberg's theorem requires that $e^{\varrho s} x_0(t + s)$ is continuous in $s$ for all $t \in (-\infty, t_0]$ and some value of $\varrho \in \Rp$, which is the case since $x_0$ is continuous by assumption. Furthermore, it requires that $e^{\varrho s} x_0(t + s) \rightarrow 0$ as $s \rightarrow -\infty$ for all $t \in (-\infty, t_0]$, which follows from the exponential boundedness of $x_0$:
%
\begin{align}
	\|e^{\varrho s} x_0(t + s)\|_\infty &= e^{\varrho s} \|x_0(t + s)\|_\infty \leq e^{\varrho s} \chmthree{L_0} e^{-\sigma (t + s)} = \chmthree{L_0} e^{-\sigma t} e^{(\varrho - \sigma) s} \rightarrow 0
\end{align}
%
as $s \rightarrow -\infty$. It is also required that $\sup_{s \in (-\infty, t]} e^{\varrho s} \|x_0(t + s)\|_\infty < \infty$ for all $t \in (-\infty, t_0]$, which also follows from the exponential boundedness:
%
\begin{align}
	\sup_{s \in (-\infty, t]} e^{\varrho s} \|x_0(t + s)\|_\infty \leq \sup_{s \in (-\infty, t]} \chmthree{L_0} e^{-\sigma t} e^{(\varrho - \sigma) s} = \chmthree{L_0} e^{-\sigma t} e^{(\varrho - \sigma) t} = \chmthree{L_0} e^{(\varrho - 2 \sigma) t}.
\end{align}
%
Finally, the norm of the measure, $\mu$, must be finite, where the norm is defined as $\|\mu\|_{\varrho} = \int_0^\infty e^{\varrho s} \|\mu(\incr s)\|_\infty$, and it is given by
%
\begin{align}
	\|\mu\|_\varrho
	&= \int_0^\infty e^{\varrho s} \|\mu(\mathrm ds)\|_\infty
	 = \int_0^\infty e^{\varrho s} \|\eta(s)\|_\infty \incr s
	 = \int_0^\infty e^{\varrho s} \|F \delta(s) + G \alpha(s) H\|_\infty \incr s \\
	&\leq \|F\|_\infty \int_0^\infty e^{\varrho s} \delta(s) \incr s + \|G\|_\infty \int_0^\infty e^{\varrho s} \|\alpha(s)\|_\infty \incr s \|H\|_\infty \nonumber \\
	&\leq \|F\|_\infty + \|G\|_\infty \int_0^\infty e^{\varrho s} L e^{-\rho s} \incr s \|H\|_\infty \nonumber \\
	&= \|F\|_\infty + L \|G\|_\infty \int_0^\infty e^{(\varrho - \rho) s} \incr s \|H\|_\infty. \nonumber
\end{align}
%
Here, $L$ is the largest amplitude in the exponential bounds on the elements of $\alpha$, and the norm is finite because $\varrho < \rho$ by assumption.}

